Beam test of a baseline vertex detector prototype for CEPC

The Circular Electron Positron Collider (CEPC) has been proposed to enable more thorough and precise measurements of the properties of Higgs, W, and Z bosons, as well as to search for new physics. In response to the stringent performance requirements of the vertex detector for the CEPC, a baseline vertex detector prototype was tested and characterized for the first time using a 6 GeV electron beam at DESY II Test Beam Line 21. The baseline vertex detector prototype is designed with a cylindrical barrel structure that contains six double-sided detector modules (ladders). Each side of the ladder includes TaichuPix-3 sensors based on Monolithic Active Pixel Sensor (MAPS) technology, a flexible printed circuit, and a carbon fiber support structure. Additionally, the readout electronics and the Data Acquisition system were also examined during this beam test. The performance of the prototype was evaluated using an electron beam that passed through six ladders in a perpendicular direction. The offline data analysis indicates a spatial resolution of about 5 um, with detection efficiency exceeding 99 % and an impact parameter resolution of about 5.1 um. These promising results from this baseline vertex detector prototype mark a significant step toward realizing the optimal vertex detector for the CEPC.

==> Achitecture.tex <==
The tested vertex detector prototype consists of three layers of concentric barrels positioned at radii ranging from \SI{18.7}{\mm} to \SI{60.5}{\mm} from the center of the cylinder. Six ladders are installed along a certain diameter direction, as shown in Fig.~\ref{fig:VTXD}\subref{fig:Picture_prototype}. The spacing and angles between each ladder plane exhibit variations, as described in~\cite{Fu2022MechanicalDO}. Each ladder is about \SI{553}{\mm} in length with a double-sided structure, consisting of two flexible printed circuit boards (PCB) supported by a carbon fiber strip as shown in Fig.~\ref{fig:VTXD}\subref{fig:Picture_ladder}. The TaichuPix-3 chip, produced with a \SI{180}{\nm} CMOS Imaging Sensor (CIS) technology, has dimensions of \qtyproduct{2.57x1.59}{\cm} and contains 1024 columns $\times$ 512 rows with a pixel pitch of \qtyproduct{25x25}{\um}. The thickness of TaichuPix-3 chip is \SI{150}{\um}. On each side of the ladder, two TaichuPix-3 chips are wire-bonded onto the end of the flexible PCB. This is because the maximum area that can be covered by the collimator provided by DESY is \qtyproduct{2.5x2.5}{\cm}. The thickness of the ladder is about \SI{3.67}{\mm}. In total, 24 chips are assembled across the six ladders.

\begin{figure}[ht]
    \begin{center}
    \subfigure[]{\includegraphics[width=0.2\textwidth]{Figures/Picture_prototype.png}\label{fig:Picture_prototype}}
    \subfigure[]{\includegraphics[width=0.27\textwidth]{Figures/Picture_ladder.pdf}\label{fig:Picture_ladder}}

    \caption{\subref{fig:Picture_prototype} Structure of the baseline vertex detector prototype; \subref{fig:Picture_ladder} detector module, also known as ladder.}
    \label{fig:VTXD}
    \end{center}
\end{figure}
